Instruction Induction: From Few Examples to Natural Language Task Descriptions

Large language models are able to perform a task by conditioning on a few input-output demonstrations - a paradigm known as in-context learning. We show that language models can explicitly infer an underlying task from a few demonstrations by prompting them to generate a natural language instruction that fits the examples. To explore this ability, we introduce the instruction induction challenge, compile a dataset consisting of 24 tasks, and define a novel evaluation metric based on executing the generated instruction. We discover that, to a large extent, the ability to generate instructions does indeed emerge when using a model that is both large enough and aligned to follow instructions; InstructGPT achieves 65.7% of human performance in our execution-based metric, while the original GPT-3 model reaches only 9.8% of human performance. This surprising result suggests that instruction induction might be a viable learning paradigm in and of itself, where instead of fitting a set of latent continuous parameters to the data, one searches for the best description in the natural language hypothesis space.

==> 05a_instructions_f1_tab.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Task} & \textbf{Human$^*$} & \textbf{davinci} & \textbf{davinci-inst}\\
\midrule
First Letter & 72.6 & 12.8 & 77.5 \\
Second Letter & 70.2 & 10.7 & 51.4 \\
List Letters & 42.6 & 21.2 & 29.6 \\
Starting With & 58.2 & 14.3 & 31.7 \\
\midrule
Pluralization & 67.0 & 29.0 & 30.2 \\
Passivization & 63.1 & 24.5 & 30.5 \\
\midrule
Negation & 38.9 & 29.4 & 38.8 \\
\midrule
Antonyms & 55.8 & 32.4 & 31.2 \\
Synonyms & 56.8 & 29.6 & 43.1 \\
Co-hyponyms & 61.0 & 19.4 & 29.7 \\
\midrule
Rhymes & 80.0 & 23.2 & 35.1 \\
\midrule
Larger Animal & 54.3 & 11.0 & 47.8 \\
\midrule
Cause Identification & 32.9 & 27.5 & 33.2 \\
Common Concept & 42.7 & 10.0 & 30.3 \\
\midrule
Formality & 53.9 & 29.1 & 30.8 \\
\midrule
Translation en-de & 76.0 & 14.7 & 44.8 \\
Translation en-es & 58.3 & 3.7 & 44.4 \\
Translation en-fr & 54.0 & 17.6 & 53.9 \\
\midrule
Sum & 44.3 & 28.3 & 46.9 \\
Diff & 70.6 & 12.8 & 73.0 \\
Number To Word & 57.8 & 30.9 & 79.2 \\
\midrule
Average & 57.7 & 20.6 & 43.5 \\
\bottomrule
\end{tabular}
\caption{instructions f1 \todo{ add categories column + bold stuff + Caption}}
\label{tab:instructions_f1}
\end{table}

==> 05b_instructions_bertscore_tab.tex <==
% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{@{}lrrr@{}}
% \toprule
% \textbf{Task} & \textbf{Human$^*$} & \textbf{davinci} & \textbf{davinci-inst}\\
% \midrule
% First Letter & 72.5 & 4.8 & 65.8 \\
% Second Letter & 71.4 & 7.8 & 58.0 \\
% List Letters & 44.7 & 21.1 & 41.0 \\
% Starting With & 52.3 & 6.0 & 35.9 \\
% \midrule
% Pluralization & 55.3 & 11.7 & 28.3 \\
% Passivization & 53.5 & 12.1 & 38.8 \\
% \midrule
% Negation & 50.5 & 26.3 & 39.4 \\
% \midrule
% Antonyms & 60.5 & 17.8 & 37.7 \\
% Synonyms & 58.6 & 20.1 & 53.2 \\
% Co-hyponyms & 45.1 & 11.4 & 30.4 \\
% \midrule
% Rhymes & 74.2 & 18.1 & 34.5 \\
% \midrule
% Larger Animal & 54.8 & 5.7 & 42.1 \\
% \midrule
% Cause Identification & 39.0 & 15.7 & 21.6 \\
% Common Concept & 50.6 & 4.3 & 24.2 \\
% \midrule
% Formality & 63.1 & 22.8 & 44.1 \\
% \midrule
% Translation en-de & 64.8 & 19.6 & 48.9 \\
% Translation en-es & 55.5 & 10.3 & 50.5 \\
% Translation en-fr & 52.0 & 19.3 & 53.4 \\
% \midrule
% Sum & 49.2 & 34.2 & 60.2 \\
% Diff & 70.1 & 8.8 & 71.1 \\
% Number To Word & 54.9 & 33.9 & 77.9 \\
% \midrule
% Average & 56.8 & 15.8 & 45.6 \\
% \bottomrule
% \end{tabular}
% \caption{instructions bert-score-f1 (deberta-xlarge-mnli) normalized. Multiplpy by 100 and increase precision? \todo{ add categories column + bold stuff + Caption}}
% \label{tab:instructions_bert_score_f1}
% \end{table}

==> 05d_execution_acc_tab.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
& \multicolumn{3}{c}{\textbf{BERTScore}} & &  \multicolumn{3}{c}{\textbf{Execution}} \\
\addlinespace[4pt]
\cmidrule(lr){2-4} \cmidrule(lr){6-8} \\
\textbf{Task} & \textbf{GPT3} & \textbf{InstructGPT} & \textbf{Human} &  & \textbf{GPT3} & \textbf{InstructGPT} & \textbf{Human}\\
\midrule
First Letter & 4.8 & 65.8 & 72.5 &  & 2.4 & 91.7 & 100.0 \\
Second Letter & 7.8 & 58.0 & 71.4 &  & 0.5 & 22.6 & 77.3 \\
List Letters & 21.1 & 41.0 & 44.7 &  & 0.1 & 3.0 & 85.4 \\
Starting With & 6.0 & 35.9 & 52.3 &  & 0.6 & 15.2 & 34.5 \\
\midrule
Pluralization & 11.7 & 28.3 & 55.3 &  & 0.0 & 97.7 & 100.0 \\
Passivization & 12.1 & 38.8 & 53.5 &  & 20.4 & 1.5 & 99.9 \\
\midrule
Negation & 26.3 & 39.4 & 50.5 &  & 6.2 & 48.7 & 70.1 \\
\midrule
Antonyms & 17.8 & 37.7 & 60.5 &  & 5.1 & 17.7 & 80.0 \\
Synonyms & 20.1 & 53.2 & 58.6 &  & 0.5 & 5.6 & 11.6 \\
Co-hyponyms & 11.4 & 30.4 & 45.1 &  & 0.1 & 7.7 & 61.4 \\
\midrule
Rhymes & 18.1 & 34.5 & 74.2 &  & 7.4 & 10.3 & 49.1 \\
\midrule
Larger Animal & 5.7 & 42.1 & 54.8 &  & 5.1 & 72.3 & 93.6 \\
\midrule
Cause Identification & 15.7 & 21.6 & 39.0 &  & 10.6 & 21.8 & 58.4 \\
Common Concept & 4.3 & 24.2 & 50.6 &  & 0.7 & 3.7 & 11.1 \\
\midrule
Formality & 22.8 & 44.1 & 63.1 &  & 39.2 & 51.1 & 56.8 \\
\midrule
Translation en-de & 19.6 & 48.9 & 64.8 &  & 2.3 & 59.2 & 75.2 \\
Translation en-es & 10.3 & 50.5 & 55.5 &  & 0.5 & 72.8 & 83.5 \\
Translation en-fr & 19.3 & 53.4 & 52.0 &  & 3.5 & 59.3 & 73.2 \\
\midrule
Sum & 34.2 & 60.2 & 49.2 &  & 12.7 & 99.9 & 99.4 \\
Diff & 8.8 & 71.1 & 70.1 &  & 6.0 & 65.8 & 99.4 \\
Number To Word & 33.9 & 77.9 & 54.9 &  & 6.6 & 98.2 & 97.8 \\
\midrule
Average & 15.8 & 45.6 & 56.8 &  & 6.2 & 44.1 & 72.3 \\
\bottomrule
\end{tabular}
\caption{BERTScore and execution accuracy for the instruction-induction experiments...	\todo{complete}.}
\label{tab:induction_results}
\end{table}

==> 05f_inst_trans.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrrr@{}}
\toprule
\textbf{M}  & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F} & \textbf{G} & \textbf{H} & \textbf{I} & \textbf{J} & \textbf{K} & \textbf{L} & \textbf{M} & \textbf{N} & \textbf{O} & \textbf{P}  & \textbf{Q} & \textbf{R} & \textbf{S} & \textbf{T}  \\
\midrule
B  & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5 & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5  & 12.3 & 19.8 & 10.4 & 77.5 \\
A & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5 & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5  & 12.3 & 19.8 & 10.4 & 77.5 \\
\bottomrule
\end{tabular}
\caption{instructions f1 \todo{ add categories column + bold stuff + Caption}}
\label{tab:my_label_f1_tmp}
\end{table}

==> 09a_instructions_f1_tab_full.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Human}} & \multicolumn{4}{c}{\textbf{GPT-3}} & \multicolumn{4}{c}{\textbf{Instruct}} \\
& & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} \\
\midrule
First Letter & 72.6 & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5 \\
Second Letter & 70.2 & 23.9 & 19.8 & 17.7 & 10.7 & 10.5 & 19.4 & 8.1 & 51.4 \\
List Letters & 42.6 & 23.0 & 25.2 & 23.4 & 21.2 & 16.6 & 28.7 & 13.9 & 29.6 \\
Starting With & 58.2 & 13.3 & 13.1 & 16.8 & 14.3 & 5.3 & 10.6 & 6.9 & 31.7 \\
\midrule
Pluralization & 67.0 & 31.7 & 26.9 & 33.6 & 29.0 & 22.2 & 30.9 & 21.5 & 30.2 \\
Passivization & 63.1 & 27.7 & 20.6 & 20.9 & 24.5 & 9.5 & 20.5 & 0.1 & 30.5 \\
\midrule
Negation & 38.9 & 28.9 & 23.5 & 27.3 & 29.4 & 13.9 & 20.3 & 13.6 & 38.8 \\
\midrule
Antonyms & 55.8 & 22.9 & 20.8 & 29.4 & 32.4 & 20.0 & 18.9 & 17.1 & 31.2 \\
Synonyms & 56.8 & 23.8 & 18.3 & 27.0 & 29.6 & 18.9 & 20.8 & 14.2 & 43.1 \\
Co-hyponyms & 61.0 & 13.9 & 15.8 & 15.9 & 19.4 & 2.7 & 10.0 & 10.5 & 29.7 \\
\midrule
Rhymes & 80.0 & 20.5 & 16.2 & 24.7 & 23.2 & 15.3 & 14.7 & 11.1 & 35.1 \\
\midrule
Larger Animal & 54.3 & 0.5 & 0.9 & 14.9 & 11.0 & 5.0 & 0.3 & 8.5 & 47.8 \\
\midrule
Cause Identification & 32.9 & 7.9 & 8.7 & 15.2 & 27.5 & 8.9 & 12.3 & 9.5 & 33.2 \\
Common Concept & 42.7 & 10.5 & 15.7 & 22.9 & 10.0 & 11.2 & 6.4 & 11.7 & 30.3 \\
\midrule
Formality & 53.9 & 14.6 & 17.8 & 14.8 & 29.1 & 4.4 & 11.9 & 5.7 & 30.8 \\
\midrule
Translation en-de & 76.0 & 22.5 & 19.1 & 15.9 & 14.7 & 15.1 & 24.5 & 7.7 & 44.8 \\
Translation en-es & 58.3 & 1.0 & 3.6 & 0.8 & 3.7 & 6.2 & 0.3 & 2.7 & 44.4 \\
Translation en-fr & 54.0 & 27.6 & 18.9 & 19.0 & 17.6 & 18.0 & 23.5 & 8.5 & 53.9 \\
\midrule
Sum & 44.3 & 28.2 & 29.8 & 34.8 & 28.3 & 24.1 & 28.4 & 42.0 & 46.9 \\
Diff & 70.6 & 15.2 & 21.8 & 30.8 & 12.8 & 32.3 & 15.6 & 23.3 & 73.0 \\
Number to Word & 57.8 & 28.3 & 28.6 & 40.1 & 30.9 & 33.0 & 28.2 & 27.8 & 79.2 \\
\midrule
Average & 57.7 & 19.5 & 18.4 & 22.4 & 20.6 & 14.5 & 17.4 & 13.1 & 43.5 \\
\bottomrule
\end{tabular}
\caption{instructions f1 \todo{ add categories column + bold stuff + Caption}}
\label{tab:my_label_f1}
\end{table}

==> 09b_instructions_bertscore_tab_full.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\textbf{Task} & \textbf{Human$^*$} & \textbf{ada} & \textbf{babbage} & \textbf{curie} & \textbf{davinci} & \textbf{ada-inst} & \textbf{babbage-inst} & \textbf{curie-inst} & \textbf{davinci-inst}\\
\midrule
First Letter & 72.5 & -10.1 & -5.0 & 10.8 & 4.8 & 0.6 & -6.8 & 7.9 & 65.8 \\
Second Letter & 71.4 & -10.2 & -4.4 & 6.4 & 7.8 & 1.6 & -5.8 & 6.8 & 58.0 \\
List Letters & 44.7 & -10.0 & 3.9 & 13.7 & 21.1 & -3.3 & 0.1 & 8.2 & 41.0 \\
Starting With & 52.3 & -5.9 & 6.5 & 8.4 & 6.0 & 2.1 & 1.6 & 3.6 & 35.9 \\
Pluralization & 55.3 & -7.6 & 0.1 & 21.1 & 11.7 & 6.9 & -5.1 & 15.5 & 28.3 \\
Passivization & 53.5 & -11.1 & 12.9 & 16.6 & 12.1 & 10.0 & 15.2 & 10.3 & 38.8 \\
Negation & 50.5 & 4.1 & 7.4 & 9.0 & 26.3 & 13.5 & 8.9 & 10.9 & 39.4 \\
Antonyms & 60.5 & -8.0 & 10.7 & 18.2 & 17.8 & 6.5 & -2.6 & 10.8 & 37.7 \\
Synonyms & 58.6 & -9.0 & 10.3 & 21.5 & 20.1 & 8.3 & 4.9 & 12.2 & 53.2 \\
Co-hyponyms & 45.1 & -11.0 & -3.5 & 6.7 & 11.4 & 5.8 & -2.1 & 2.2 & 30.4 \\
Rhymes & 74.2 & -14.4 & 2.0 & 17.6 & 18.1 & 5.0 & 0.6 & 5.2 & 34.5 \\
Larger Animal & 54.8 & -8.1 & -5.5 & -4.9 & 5.7 & -3.4 & -4.3 & -0.8 & 42.1 \\
Cause Identification & 39.0 & -2.2 & 8.7 & 6.6 & 15.7 & 6.0 & 7.0 & 10.0 & 21.6 \\
Common Concept & 50.6 & -19.1 & -1.3 & 10.7 & 4.3 & -0.7 & -0.4 & 6.8 & 24.2 \\
Formality & 63.1 & -1.5 & 16.5 & 13.3 & 22.8 & 16.4 & 9.4 & 16.4 & 44.1 \\
Translation en-de & 64.8 & -5.4 & 1.0 & 12.1 & 19.6 & 5.9 & -4.6 & 10.4 & 48.9 \\
Translation en-es & 55.5 & -10.0 & -1.9 & -3.0 & 10.3 & -2.7 & -6.0 & 6.4 & 50.5 \\
Translation en-fr & 52.0 & -1.0 & 11.7 & 8.9 & 19.3 & 3.9 & 5.7 & 11.4 & 53.4 \\
Sum & 49.2 & -12.2 & 8.3 & 25.8 & 34.2 & 15.6 & -12.1 & 41.9 & 60.2 \\
Diff & 70.1 & -17.3 & 6.1 & 23.4 & 8.8 & 14.2 & -17.3 & 26.4 & 71.1 \\
Number To Word & 54.9 & -2.4 & -2.3 & 28.0 & 33.9 & 13.8 & -1.8 & 30.0 & 77.9 \\
\midrule
Average & 56.8 & -8.2 & 3.9 & 12.9 & 15.8 & 6.0 & -0.7 & 12.0 & 45.6 \\
\bottomrule
\end{tabular}
\caption{instructions bert-score-f1 (deberta-xlarge-mnli) normalized. Multiplpy by 100 and increase precision? \todo{ add categories column + bold stuff + Caption}}
\label{tab:instructions_bert_score_f1_all_models}
\end{table}

==> 09c_in_context_tab_full.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\textbf{Task} & \textbf{ada} & \textbf{babbage} & \textbf{curie} & \textbf{davinci} & \textbf{ada-inst} & \textbf{babbage-inst} & \textbf{curie-inst} & \textbf{davinci-inst}\\
\midrule
First Letter & 79.0 & 96.0 & 99.0 & 97.0 & 66.0 & 91.0 & 96.0 & 98.0 \\
Second Letter & 8.0 & 9.0 & 16.0 & 25.0 & 8.0 & 9.0 & 5.0 & 34.0 \\
List Letters & 7.0 & 35.0 & 69.0 & 98.0 & 2.0 & 30.0 & 59.0 & 100.0 \\
Starting With & 11.0 & 16.0 & 21.0 & 33.0 & 6.0 & 13.0 & 19.0 & 46.0 \\
Pluralization & 73.0 & 89.0 & 95.0 & 95.0 & 75.0 & 88.0 & 95.0 & 99.0 \\
Passivization & 78.0 & 95.0 & 97.0 & 100.0 & 81.0 & 91.0 & 96.0 & 100.0 \\
Negation & 58.0 & 87.0 & 93.0 & 94.0 & 56.0 & 80.0 & 84.0 & 93.0 \\
Antonyms & 37.0 & 66.0 & 75.0 & 84.0 & 35.0 & 55.0 & 78.0 & 83.0 \\
Synonyms & 2.0 & 4.0 & 5.0 & 9.0 & 0.0 & 6.0 & 9.0 & 12.0 \\
Co-hyponyms & 3.0 & 6.0 & 11.0 & 13.0 & 2.0 & 1.0 & 0.0 & 36.0 \\
Rhymes & 32.0 & 69.0 & 63.0 & 46.0 & 2.0 & 6.0 & 8.0 & 39.0 \\
Larger Animal & 49.0 & 60.0 & 64.0 & 58.0 & 51.0 & 52.0 & 45.0 & 82.0 \\
Cause Identification & 54.0 & 41.0 & 53.0 & 45.0 & 57.0 & 52.0 & 50.0 & 76.0 \\
Common Concept & 11.8 & 18.5 & 16.7 & 22.9 & 13.4 & 13.9 & 14.6 & 15.2 \\
Formality & 39.1 & 45.6 & 50.4 & 54.4 & 34.2 & 44.1 & 46.6 & 56.4 \\
Translation en-de & 23.0 & 59.0 & 69.0 & 80.0 & 13.0 & 35.0 & 64.0 & 85.0 \\
Translation en-es & 31.0 & 58.0 & 73.0 & 91.0 & 17.0 & 50.0 & 72.0 & 88.0 \\
Translation en-fr & 34.0 & 54.0 & 67.0 & 80.0 & 29.0 & 44.0 & 68.0 & 84.0 \\
Sum & 3.0 & 0.0 & 6.0 & 87.0 & 1.0 & 3.0 & 11.0 & 100.0 \\
Diff & 3.0 & 2.0 & 4.0 & 69.0 & 2.0 & 1.0 & 5.0 & 95.0 \\
Number To Word & 0.0 & 44.0 & 74.0 & 85.0 & 5.0 & 28.0 & 69.0 & 100.0 \\
\midrule
Average & 30.3 & 45.4 & 53.4 & 65.1 & 26.5 & 37.8 & 47.3 & 72.5 \\
\bottomrule
\end{tabular}
\caption{in-context score \todo{ add categories column + bold stuff + Caption}}
\label{tab:in_context_score_all_models}
\end{table}

==> 10_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \S\ref{sec:ambiguity} and the comment regarding the execution model in \S\ref{sec:results_execution}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
     \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include our data as well as model predictions. Our code will be made publicly available upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We didn't perform any training, only inference, for which we reported the inference settings, see \S\ref{sec:results}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{We cited the assets and provided necessary links, license details can be found there. All datasets used are open and publicly available.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{No such danger in our data.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See \S\ref{sec:annotations} and \S\ref{sec:verification}.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{The annotations were very limited in scope (a few minutes of work from each annotator), which we got via personal friends who were not involved in the project.}
\end{enumerate}


\end{enumerate}


==> old_omer_table.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Human}} & \multicolumn{4}{c}{\textbf{GPT-3}} & \multicolumn{4}{c}{\textbf{Instruct}} \\
& & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} \\
\midrule
First Letter & 72.6 & 24.5 & 20.6 & 24.0 & 12.8 & 12.3 & 19.8 & 10.4 & 77.5 \\
Second Letter & 70.2 & 23.9 & 19.8 & 17.7 & 10.7 & 10.5 & 19.4 & 8.1 & 51.4 \\
List Letters & 42.6 & 23.0 & 25.2 & 23.4 & 21.2 & 16.6 & 28.7 & 13.9 & 29.6 \\
Starting With & 58.2 & 13.3 & 13.1 & 16.8 & 14.3 & 5.3 & 10.6 & 6.9 & 31.7 \\
\midrule
Pluralization & 67.0 & 31.7 & 26.9 & 33.6 & 29.0 & 22.2 & 30.9 & 21.5 & 30.2 \\
Passivization & 63.1 & 27.7 & 20.6 & 20.9 & 24.5 & 9.5 & 20.5 & 0.1 & 30.5 \\
\midrule
Negation & 38.9 & 28.9 & 23.5 & 27.3 & 29.4 & 13.9 & 20.3 & 13.6 & 38.8 \\
\midrule
Antonyms & 55.8 & 22.9 & 20.8 & 29.4 & 32.4 & 20.0 & 18.9 & 17.1 & 31.2 \\
Synonyms & 56.8 & 23.8 & 18.3 & 27.0 & 29.6 & 18.9 & 20.8 & 14.2 & 43.1 \\
Co-hyponyms & 61.0 & 13.9 & 15.8 & 15.9 & 19.4 & 2.7 & 10.0 & 10.5 & 29.7 \\
\midrule
Rhymes & 80.0 & 20.5 & 16.2 & 24.7 & 23.2 & 15.3 & 14.7 & 11.1 & 35.1 \\
\midrule
Larger Animal & 54.3 & 0.5 & 0.9 & 14.9 & 11.0 & 5.0 & 0.3 & 8.5 & 47.8 \\
\midrule
Cause Identification & 32.9 & 7.9 & 8.7 & 15.2 & 27.5 & 8.9 & 12.3 & 9.5 & 33.2 \\
Common Concept & 42.7 & 10.5 & 15.7 & 22.9 & 10.0 & 11.2 & 6.4 & 11.7 & 30.3 \\
\midrule
Formality & 53.9 & 14.6 & 17.8 & 14.8 & 29.1 & 4.4 & 11.9 & 5.7 & 30.8 \\
\midrule
Translation en-de & 76.0 & 22.5 & 19.1 & 15.9 & 14.7 & 15.1 & 24.5 & 7.7 & 44.8 \\
Translation en-es & 58.3 & 1.0 & 3.6 & 0.8 & 3.7 & 6.2 & 0.3 & 2.7 & 44.4 \\
Translation en-fr & 54.0 & 27.6 & 18.9 & 19.0 & 17.6 & 18.0 & 23.5 & 8.5 & 53.9 \\
\midrule
Sum & 44.3 & 28.2 & 29.8 & 34.8 & 28.3 & 24.1 & 28.4 & 42.0 & 46.9 \\
Diff & 70.6 & 15.2 & 21.8 & 30.8 & 12.8 & 32.3 & 15.6 & 23.3 & 73.0 \\
Number to Word & 57.8 & 28.3 & 28.6 & 40.1 & 30.9 & 33.0 & 28.2 & 27.8 & 79.2 \\
\midrule
Average & 57.7 & 19.5 & 18.4 & 22.4 & 20.6 & 14.5 & 17.4 & 13.1 & 43.5 \\
\bottomrule
\end{tabular}
\caption{instructions f1 \todo{ add categories column + bold stuff + Caption}}
\label{tab:my_label_f1}
\end{table}
